Bayesian sampling with BeAtlas, a grid of synthetic Be star spectra I. Recovering the fundamental parameters of \alpha Eri and \beta CMi

Classical Be stars are fast rotating, near main sequence B-type stars. The rotation and the presence of circumstellar discs profoundly modify the observables of active Be stars. Our goal is to infer stellar and disc parameters, as well as distance and interstellar extinction, using the currently most favoured physical models for these objects. We present BeAtlas, a grid of 61.600 NLTE radiative transfer models for Be stars, calculated with the HDUST code. The grid was coupled with a Monte Carlo Markov chain code to sample the posterior distribution. We test our method on two well-studied Be stars, $\alpha$ Eri and $\beta$ CMi, using photometric, polarimetric and spectroscopic data as input to the code. We recover literature determinations for most of the parameters of the targets, in particular the mass and age of $\alpha$ Eri, the disc parameters of $\beta$ CMi, and their distances and inclinations. The main discrepancy is that we estimate lower rotational rates than previous works. We confirm previously detected signs of disc truncation in $\beta$ CMi and note that its inner disc seems to have a flatter density slope than its outer disc. The correlations between the parameters are complex, further indicating that exploring the entire parameter space simultaneously is a more robust approach, statistically. The combination of BeAtlas and Bayesian-MCMC techniques proves successful, and a powerful new tool for the field: the fundamental parameters of any Be star can now be estimated in a matter of hours or days.

==> DISCUSSION_OLD.tex <==
\section{Discussion}

In this section we discuss the results of all simulations for all three targets. We compare the PDFs obtained by each of our simulations and define what the ``final'' result for the parameter values for our targets is. We then compare those results with previously published determinations. We also discuss the low values of $n$ ($n$ < 3.5) found for all three targets, and the prevalence of disk truncation.


\subsection{Selecting the final result}

\beatlas is a grid of physical models of Be stars constructed using the \hdust radiative transfer code and the Geneva grid of evolutionary models for fast rotators, using the steady-state, isothermal approximation of the VDD model. It is therefore very much dependent on the physics on which \hdust and the Geneva grid are built. Different observables are also not just coming from different parts and areas of the disk (see Sect. XX), but are also created by entirely different physical processes between the starlight and the disk particles. Thus, it was expected that the results for the parameters would not be the same for all observables. Our intention here was to look at the problem from many angles and find if there was a combination of parameter values that could sufficiently describe all observations.

It is then remarkable that for all three targets the result for the base density of the disk (log $n_0$) derived using the SED is basically the same as the value found using the polarisation. One observable is caused by absorption and re-emission of light, while the other comes from scattered light in the inner disk, and both agree on the $XX$ $cm^{-2}$. The same can be said for the inclination, which in one case comes from measurements of He I and Mg II lines (via our prior on \vsini), and on the other from the polarisation.

\ACR{In other cases, such as for the density exponent of \acol, the discrepancy in the results of the SED versus the polarisation helps us discriminate between the two solutions given by the SED simulation.}

Simulations for different observables sometimes also provided different results. In order to compare our findings with previous determinations of parameters for the targets, we must define what are our ``final'' results for the parameters of our targets. We approach this in two ways: multiplying the PDFs derived by the two different simulations to find their ``common'' most likely values for the parameters; and analyse the individual results by their physical possibility, case by case. 

\ACR{Preciso ter todos os modelos pra fazer isso}

\begin{table}
    \centering
    \caption{Inferred and derived parameters for all targets.}
    \begin{tabular}{c c c c c c}
    \hline
    \hline
    & \bcmi & \acol & \aara \\
    \hline
    $M\, [\mathrm{M_\odot}]$ \\
    $\log \, n_0$ \\
    $\log g$ \\
    $R_\mathrm{D}\, [\mathrm{R_\star}]$ \\ 
    $R_\mathrm{pole}\, [\mathrm{R_\odot}]$ \\ 
    $n$ \\ 
    $L\, [\mathrm{L_\odot]}$ \\ 
    $i$ $[\mathrm{^o}]$ \\ 
    $T_\mathrm{eff}\,[\mathrm{K}]$ \\
    $d\, [\mathrm{pc}]$ \\
    $W$ \\
    $\beta_\mathrm{GD}$ \\
    $t/t_\mathrm{MS}$ \\ 
    $E(B-V)\, \mathrm{[mag]}$\\ 
    \hline
    \end{tabular}
    \label{tab:best_fit}
\end{table}



\subsection{\halp profiles}

The \beatlas grid also has \hdust calculated \halp profiles in addition to SEDs and polarisation for the lower mass end of CBes. Thus, can we compare the profiles derived from our SED+polarisation result to literature spectra for the late-types \bcmi and \acol. 

As detailed in Sect. \ref{sec:methodology}, the EW of the \halp line is used as a prior for the MCMC simulation of the SED for these two targets. As the result for the stellar parameters of this simulation is then used as prior for the polarisation MCMC, then this EW prior is relevant for results of both simulations. 

\hdust does not include line wing broadening by non-coherent electron scattering. Following \citet{marr2021}, this effect is artificially added by convolving the synthetic line profile of our ``best fit'' result with a Gaussian that has a FWHM of the thermal velocity of the scattered electrons.

In Fig. QUE AINDA NAO EXISTE shows the comparison between the observed \halp line profiles of the \bcmi and \acol with the artificially broadened results of a random selection of our sampled simulations for the SED (in COLOR) and polarisation (in COLOR), and also for our general best fit model from Table \ref{tab:best_fit} (in COLOR). 



\subsection{Comparing with literature}

\ACR{RECHECK ALL VALUES}
\subsubsection{\bcmi}
A comparison of our best-fit parameters with those of \cite{klement2015, klement2017} (Tab. \ref{tab:bcmi_parameters}) shows an agreement for some parameters but a discrepancy for others. From now on, we refer to the results of \citeauthor{klement2015} as K15. Before any comparison, we review the main differences between our approach and that used by K15: both the stellar parameters, the inclination and the extinction are fixed in K15, while they are free on ours; the ranges of the free parameters are also larger in \beatlas; their best-fit results are based on a manual, $\chi^2$ based search, while ours are based on the credible interval of the PDF defined by MCMC sampling. 

Our estimate of the equatorial radius and rotation rate match previous interferometric studies of \citet[$R_\mathrm{eq} = 3.6 \,  \mathrm{R_\odot}$]{quirrenbach1997} and \citet[$W = 0.85 \pm 0.21$; $R_\mathrm{eq} =  3.6 \pm 0.3 \,  \mathrm{R_\odot}$]{tycner2005} but differ from K15. This is likely due to the discrepancy in mass between our inference and K15, given the fact that our inferred $E(B-V)$ is larger than their fixed value. It is worth noting that our results for the mass are in agreement with those of \citet[$3.8 \, \mathrm{M_\odot}$]{2013A&A...550A..79C} and \citet[$3.5 \pm 0.2 \, \mathrm{M_\odot}$]{fremat2005}.

The inclination angle is in good agreement, as well as with the values determined by \citet[$54.5 \pm 2.9\degree$]{fremat2005} and \citet[$38.5 \pm 1.0\degree$]{2012ApJ...744...19K}. The close match of our value of $i$ and those of Kraus et al. [CITAÇÃO??] and K15 is a quite significant result, since our model used only the SED and the polarisation, while the other determinations relied on interferometric measurements, which is quite sensitive to $i$. Most likely this is a direct result of our use of literature \vsini as a prior. Finally, our estimate for the age in the MS is in agreement with previous determinations (e.g. \citealp{2005A&A...441..235Z}; \citealp{2006MNRAS.371..252L}) suggesting that \bcmi is in the second half of its MS lifetime.

% n and rho0
As for disk, we found $n = 2.44^{+0.27}_{-0.16}$ and $\log n_0 = 11.99^{+0.21}_{-0.10}$ in good agreement with K15. According to \cite{vieira2017}, these are typical values for Galactic late-type CBes (see their Fig. 7). The relatively low value of $n$ deserves some further comments. Since \bcmi has a stable disk, and because isothermal steady-state discs have a density slope of $n=3.5$ \citep{bjorkman2005}, we speculate two possible causes for the low $n$: 1) Accumulation effect caused by a binary companion (see Sect. \ref{sect:introduction} and \citealt{panoglou2016}); 2) Non-isothermal effects in the disk, that may cause a shallower profile \citep{carciofi2008}. This is discussed in more depth in Sect. XX.

Figure \ref{sed_bcmi} shows the full SED of \bcmi, together with our best-fit model and the reference model. The SED turndown is easily seen near 1 mm, and both models seem to reproduce it well, which is expected given the rough agreement between the inferred values of the disk radius, $R_\mathrm{D}$, for both cases.

\ACR{ISSO AINDA É VÁLIDO?? PRECISO DO MODELO FINAL PRA DIZER.\\
A comparison between the residuals shows some interesting features. Our best fit model clearly performs better in the UV up to the far-IR regions than in longer wavelengths. For the reference model, the residuals are systematically offset to positive values and have a negative slope. Both these facts indicate that the stellar mass may have been underestimated by the reference model. This further corroborates the larger mass found in our study. On the other hand, the reference model performed much better in the microwave region of the SED. One possible reason for this lies in the modelling procedure adopted by \citeauthor{klement2015} (op. cit.), which focused on the long-wavelength SED when manually searching for the best parameters. }


% Summary plot
\begin{figure*}
\centering
\includegraphics[width=1.\linewidth]{figures/bcmi.pdf}
\caption{Upper panel: SED of \bcmi showing the best-fit \beatlas model (black solid line) and the reference model of \cite{2017A&A...601A..74K}. The spectral regions are highlighted in order to facilitate the identification of the adopted spectral regions. Inset: A zoom to the UV up to the \texttt{NIR} region. Lower panel: residuals of the best-fit \beatlas models (black dots) and of the reference model (circles).  VC LEMBRA PRA Q Q ERA ESSE LEMBRETE, ALEX??
\textcolor{red}{ALEX: check Robert's email April, 27th,2020}
}

\label{sed_bcmi}
\end{figure*}


% MUDAR ESSE PARÁGRAFO E COLOCAR DEPOIS DE AARA, FALANDO DAS 3 ESTRELAS AO MESMO TEMPO
% Overall, our \beatlas + Bayesian-MCMC approach to the problem of inferring the fundamental parameters of the CBe star \bcmi successfully addressed the issues presented in Sect. \ref{sect:introduction}. We were able explore the entire SED and the optical polarization, providing a self-consistent simultaneous determination of the stellar and disk parameters. The usage of MCMC techniques ensures that the errors of each parameter are properly propagated to all others, and also allows for the quantification of the correlations between the various parameters. A final remark is that our result, once the \beatlas grid was ready and all the routines written and tested, was produced in a matter of hours, instead of the months taken by R. Klement for this manual search of the parameter space. This demonstrates that \beatlas + MCMC offers an ideal solution for the quick analysis of large samples of CBes. 

\subsubsection{\acol}
RECHECK VALUES AND REWRITE
Differently from \bcmi, \acol was never the target of a in-depth research before, but there are some measurements mainly of its stellar and geometrical parameters to be found in literature. 

Our final result is given in Table \ref{tab:best_fit}. The stellar mass of $4.68_{-0.09}^{+0.12}\, M_{\odot}$ agrees with the determination of \citet{chauville2001} and \citet{zorec2016} within the uncertainties. The rotation rate of $0.74_{-0.06}^{+0.06}$ indicates a $R_{eq}/R_{\rm pole} = 1.27\pm 0.2$. Interpolating the values derived for the mass, $W$, and age with the Geneva evolutionary model grid, we find a log luminosity of $\approx 2.95$, agreeing within 1 $\sigma$ with the determination of \citet{levenhagen2006} and \citet{zorec2012}; an $R_{eq} \approx 6.46\pm0.5 \, R_{\odot}$, which does not quite agree with the determination of \citet{arcos2018} and \citet{meilland2012}, but is compatible within 3 $\sigma$, and an $R_{\rm pole} \approx 5.23\pm 0.3 \, R_{\odot}$. From these values, we derive a $v_{\rm crit} \approx 341.60\pm10.0$ km/s, in accordance to the values derived by \citet{zorec2005, zorec2016} from their analysis of \acol's spectral lines in 1 $\sigma$. From $W$ we can also derive the rotational velocity of the star as $v_{rot} \approx 275.12$ km/s. Combining this result with our determination of the inclination, we find a resulting $v\sin(i)$ of 174.46 km/s, similar to the determinations of \citet{levenhagen2006}, \citet{zorec2012} and \citet{zorec2016} within 1 $\sigma$. The value of $t/t_{\rm MS} = 0.95_{-0.02}^{+0.01}$ indicates that the star is evolved, at the very end its main sequence lifetime. In newer versions of \beatlas, the possibility of expanding the study stars just past MS ($t/t_{\rm MS} >$ 1) like \acol will be possible. Finally, it is interesting to note that most of these literature parameter determinations comes from spectral line analysis, while in our work we only considered photometry, polarimetry and UV spectroscopy, but no in-depth line analysis, and still recovered most of the values determined by these studies.

% \begin{table}[]
%     \centering
%     \begin{tabular}{ll}
%         \hline
%          Parameter & Value \\
%          \hline
%          Mass [$M_{\odot}$] & $4.68_{-0.09}^{+0.12}$ \\
%          Rotation Rate & $0.74_{-0.06}^{+0.06}$\\
%          Age & $0.95_{-0.02}^{+0.01}$\\
%          Log disk Base Density [cm$^{-3}$] & $11.96_{-0.07}^{+0.14}$ \\
%          disk Radius [$R_{eq}$] & $19.89_{-5.7}^{+2.3}$ \\
%          disk Density Exponent & $2.50_{-0.09}^{+0.29}$\\
%          Inclination [$\degree$] & $41.78_{-5.1}^{+5.7}$\\
%          Distance [pc] & $79.84_{-2.2}^{+2.2}$ \\
%          Extinction & $0.023_{-0.005}^{+0.005}$\\
%          $R_{eq}/R_{\rm pole}$ & $1.27\pm 0.2$\\
%          $R_{eq}$ [$R_{\odot}$] &  $6.46\pm0.5$ \\
%          $R_{\rm pole}$ [$R_{\odot}$] & $ 5.23\pm 0.3$ \\
%          $v_{\rm crit}$ [km/s] & $341.60\pm10.0$\\
%          \hline
%     \end{tabular}
%     \caption{\footnotesize Parameter results from \textsc{bemcee} for the combination of the results for the SED and polarimetry of \acol. Distance and extinction are the same as the SED result, as these parameters are not included in the polarimetry run.}
%     \label{tab:finalresults}
% \end{table}



The disk, as expected from the low polarisation signal, is tenuous, with a log base density of $11.96_{-0.07}^{+0.14}$, corresponding to $9.08_{-1.3}^{+3.5} \times 10^{-13}$ g cm$^{-3}$, larger than the previous determination of \citet{vieira2017} of $11.51^{+0.02}_{-0.01}$. The radial density exponent sits at $n = 2.50_{-0.09}^{+0.29}$, in agreement with \citet{vieira2017} determination of $n = 2.76^{+0.04}_{-0.03}$. This is an interesting result, and was also seen for \bcmi. \citet{vieira2017} classified discs with $n \leq 3.0$ as dissipating disks (as shown in Fig. \ref{fig:rodrigo13}). However, \acol has by all means an incredibly stable disk, showing very little variation in line measurements of \halp (Fig. \ref{fig:linemeasures}) and polarisation (Fig. \ref{fig:poldata}). \ACR{The TESS light curve for \acol, covering a period of 27 days, shows no signs of outbursts or other events connected to disk variability (COLOCAR NO APÊNCIDE? Fig \ref{fig:lightcurve})}. We find no other indication that \acol has undergone a disk build-up or dissipation event since its discovery as a Be star in 1897. This is further discussed in Sect. XX.

The disk is truncated at XX \req, once again in similar fashion to \bcmi. Given this result, we searched for signals of a companion in the spectra we collected for \acol. We focused specially on looking for RV shifts and periodic V/R variations in \halp lines using Lomb-Scargle methods, as was done for \bcmi by \citet{dulaney2017}. However, as of this publication, no clear detection of a secondary was possible. This can be due to the fact that, even though many spectra were collected, a great portion of them was actually taken in the same or consecutive nights, thus making the dataset unhelpful to detect longer term shifts and variations.


\subsubsection{\aara}
Similarly to \acol, \aara was also never the target of a focused study. Therefore we compare our results with previous literature determinations. The disk parameters of \aara, $n = {2.85}_{-0.10}^{+0.25}$ and $\log n_0 = {12.87}_{-0.02}^{+0.03}$, are in agreement with the average properties of Galactic Be stars of similar spectral type \citep{2017MNRAS.464.3071V}. Our result also agrees with the affirmation that discs around early-type stars are denser (Sect. \ref{sect:introduction}). Once again the value for $n$ derived by our study is lower than the canonical value of $n=3.5$, even for a confirmed stable disk. Because the observational data established a very stable disk around \aara, the situation is similar to the case of \bcmi and \acol: the value of $n$ for stable isothermal discs may be due to non-isothermal effects, an unseen companion, or both. This is further discussed in Sect. XX.

One quite significant result from the \beatlas is that the model firmly indicates that the disk of \aara is truncated, and the truncation radius is much smaller than that of \bcmi, indicating that, if a companion is indeed responsible for the truncation, it is much closer to the CBe star than \bcmi's. Using both truncation radius and the mass we estimate roughly the period and the semi-major axis of the putative binary system. Assuming a companion with 2.0 $\mathrm{M_\odot}$ resulted in a period of $P = 34.0 \pm 9.5 \, \mathrm{days}$ for a circular coplanar orbit. Here, we applied the correction proposed by \cite{2016MNRAS.461.2616P}. \ACR{SE EU PUDER FALAR DA COMPANHEIRA Q O ROBERT ENCONTROU, ESSA DISCUSSÃO N É MAIS NECESSÁRIA. eu mudaria esse parágrafo inteiro pra fechar essa seção \\ Our values for the truncation radius and period do not agree with those of \cite{2005A&A...435..275C} ($R_\mathrm{D} = 32 \, R_\star$ and $P \sim 74 \, \mathrm{days}$) or \cite{1991A&A...241..159M} (47.5 days). It must be emphasised that both results are rough estimates of periods obtained from radial velocity measurements and $V/R$ variations. These estimates were made from data taken over a short observation period (less than two months), which clearly is not enough for a precise period determination. What can be concluded from their spectroscopic data with some confidence, however, is that the radial velocities do indicate the presence of a companion. We conclude that both our results and the spectroscopic data corroborate the hypothesis that \aara has indeed a companion, but more spectroscopic data is necessary to obtain an independent estimate of the orbital period. }

% % The final SED with the best models (stellar and system)
% The full SED of \aara is displayed in Fig. \ref{fig:sed_aara}. Shown are the best-fit model for the star itself (blue line) and the star plus disk (green dashed line). The figure has many points of interest. Examining the UV part, we see that the star + disk model lies below the purely photospheric model. This is because the disk partially absorbs some of the stellar UV flux and reprocesses it towards longer wavelengths, thus causing the large IR excess (orange-shaded area). This stresses the importance of a self-consistent analysis of the SED, including both the star and the disk. The truncation caused by the unseen companion can also be observed around $10^6\,\mathrm{\AA}$. The position of the SED turndown is not well defined, due to the lack of observations at other wavelengths.
% % routine r_truncation.py

% % Summary plot
% \begin{figure*}
% \centering
% \includegraphics[width=0.8\linewidth]{figures/sed_alf_ara.pdf}
% \caption{SED of \aara showing the best-fit photospheric model (blue line) and the star + disk model (green dashed line). The orange-shaped area shows the IR excess. The spectral regions are highlighted in order to facilitate the identification of the different spectral regions.}\label{fig:sed_aara}
% \end{figure*}

% \ACR{I DON'T LIKE THIS!!!!! VOU TIRAR QUANDO ESTIVER REVISANDO ESSA PARTE}
% The above discussion can be summarised as follows:

% \begin{itemize}
%     \item The \beatlas model of \aara was able to constrain all fitted parameters. The model includes as priors the distance and the $v \, \sin \,i$, both of which greatly narrowed the confidence intervals of the fitted parameters;

%     \item All parameters are fitted simultaneously, therefore their interdependence is properly taken into consideration;
    
%     \item The model parameters were obtained under two theoretical assumptions: 
%         \begin{enumerate}
%             \item The stellar parameters are driven by the Geneva models. Therefore, the age of the star must be analysed in this context;
            
%             \item The disk parameters reflect a power law \texttt{VDD}, and also must be analysed in this context. Considering that \aara has a stable disk,the inferred value for $n = 2.85^{+0.25}_{-0.10}$ suggests that other mechanisms may be controlling the slope of the density profile. Possibilities are binary or non-isothermal effects.
%         \end{enumerate}

%     \item A relevant result is that the independent analysis of the polarisation and the SED yielded quite consistent results for the disk parameters. This is relevant because the SED and polarisation are controlled by two very different processes;

%     \item When combined the two analysis provided a better fit of some of the parameters, specially the inclination angle;

%     \item Also noteworthy is the excellent agreement between our results and interferometric estimates for the inclination; 

%     \item Our analysis provided strong evidence of disk truncation for \aara.
   
% \end{itemize}


\subsection{Disk truncation}\label{sec:disk_truncation}


The size of the disk, $R_D$, is a parameter related to the flux emission in larger areas of the disk. Using \citet{vieira2015}'s pseudo-photosphere model, we can understand the disk of a CBe star as having two distinct parts: an inner optically thick region (the pseudo-photosphere) and an outer optically thin region, and the final flux will be a combination of the emission of these two regions. The size of the pseudo-photosphere  has a wavelength dependency. At wavelengths larger than visible, the size of the pseudo-photosphere grows, meaning that larger and larger areas of the disk contribute more to the emission. From mid-infrared onward, the disk dominates as the emitting area grows. For wavelengths were the pseudo-photosphere is small, a large part of the flux will be depleted, but if it is large, then the increased emitting area will lead to a brightening of the system. Truncating the disk at a radius smaller than the effective radius of the pseudo-photosphere affects the amount of flux emitted by the outer disk,and therefore leads to a steepening of the SED in the radio/centimetre region. Thus, the size of the disk is inferred based on the drop on emission from longer wavelengths (called SED turndown), which indicated that the emitting area of the disk is smaller. 

This feature was first observed by \citet{waters1991}, where they analyse VLA and IRAS data for 6 bright Be stars: $\gamma$ Cas, $\beta$ Mon A, $\eta$ Tau, EW Lac, $\psi$ Per, and $\beta$ CMi. $\gamma$ Cas is now famously in a binary system, but at the time none of the stars was believed to have a companion. \citeauthor{waters1991} suggest as a cause for this ``turnover'' a change in the geometry of the disk,or an additional acceleration of the material in the outer region, but in no great detail. 

Following the theory for the VDD, the disk of an isolated CBe star should in principle expand viscously until it reaches the sonic point where the radial velocity in its outermost region reaches the sound speed. Beyond this point, the disk is then in the transonic regime, where the azimuthal velocity is no longer Keplerian, but angular momentum conserving. This also leads to a change in the density profile of the disk,making it steeper \citep{okazaki2001}. The typical values for this point are about 430 \req for a B9V star and 350 \req for a B0V \citep{krticka2011}. 

For all our three targets, we derived values of $R_D$ (see Table \ref{tab:best_fit}) that are much lower than could be explained by the sonic point. Thus, our results cannot be explained in the context of an isothermal steady-state VDD disk.

There are two main possible sources for the disk truncation: non-isothermal effects, where the changes in temperature throughout the disk lead to changes in emitted flux \citep{carciofi2008}; or the presence of a companion in a close binary system, where the tidal torque exerted by this companion stops the growth of the disk, truncating it at about 0.8 of the semi-major axis of the system (\citealt{okazaki2002}, \citealt{panoglou2016}).  



The following studies of \citet{klement2017, klement2019} searched for signs of SED turndown in a larger sample of CBe stars, both known binaries and single stars. \citet{klement2017} revisited the studied of \citet{waters1991} IR data for $\gamma$ Cas, $\beta$ Mon A, $\eta$ Tau, EW Lac, $\psi$ Per, and \bcmi and confirmed the presence of SED turndown for the targets.

In \citet{klement2019}, the sample was expanded for 57 CBe stars. For 31 stars, there was not enough data to conclusively determine whether the turndown was present or not. For the remaining 26 Be stars with sufficient data to accurately interpret the slope of the long-wavelength SED, the turndown was confirmed for 100$\%$ of the cases. Hence, there is reason to believe all Be stars may be binaries, only we were unable to espy their companions until now.

Our results indicate disk sizes of X, X, and X for \bcmi, \acol, and \aara respectively. The truncation of the disk seems to indicate the presence of unseen binary companions in these systems. In the case of \bcmi, there is a likely detection of a companion (see however Sect. \ref{sect:overview_bcmi}). For \aara AAAAAA. Finally, no clear observational signals of a companion were found in our analysis of \acol's \halp spectra. Therefore, at least for our sample, the SED turndown $\longrightarrow$ companion connection cannot be confirmed.


% This result of particular importance when we recall that companions in a system with a Be star, unless they are X-ray emitters, can be quite difficult to detect. The detection of this SED turndown can then help us find these hidden binary systems.


\subsection{Prevalence of low $n$}

\ACR{Essa é a mesma discussão q está na minha dissertação. }

In recent years, other in-depth studies of individual CBe stars in using our previous versions of the \beatlas grid have been performed: $o$ Aqr \citep{almeida2019}, 66 Oph \citep{marr2021}, and of course \bcmi, \acol and \aara in this paper. For all these targets, the values for the radial density exponent $n$ were found to be well below the standard value of 3.5.


$o$ Aqr (HD 209409) is a Shell star, a Be star seen at a close to edge-on inclination. It possesses a fairly stable disk, as attested by the regularity of its \halp line measurements (\citealt{rivinius2006}, \citealt{sigut2015}). \citet{almeida2019} used visible and near-infrared CHARA/VEGA and VLTI/AMBER spectro-interferometric data of the \halp and Br$\gamma$ lines to characterise the star. Their best fit values for the base density of the disk and its radial density exponent are $\rho_0 = 5.0 \times 10^{-12}$ g cm$^{-3}$ and $n = 3.0$. An earlier study of the same star using NPOI \halp interferometric visibilities and the \textsc{bedisk} radiative transfer code \citep{sigut2007} found $\rho_0 = 6.0 \times 10^{-12}$ g cm$^{-3}$ and $n = 2.7$ \citep{sigut2015}. Neither study quoted their respective uncertainties in these values.

% $\alpha$ Ara (HD 158427) is an early type Be star, and quite close by, at $\sim$ 74.3 pc away. It was meticulously studied by \citeauthor{mota2019b} as one of the first tests for BeAtlas and \textsc{bemcee}, with observational data in photometry and polarimetry used to derive its fundamental parameters. The most likely values for the disk parameters are log $n_0 = 12.87^{+0.03}_{-0.02}$ ($\approx \rho_0 = 7.38 \times 10^{-12}$ g cm$^{-3}$) and $n = 2.85^{+0.25}_{-0.10}$.

66 Oph (HD 164284) has undergone disk build up from 1957 to 1995, so it could, during that period, be considered an active CBe star. The most recent results from the MCMC analysis with photometry and UV spectroscopy of the star indicate it had a disk with a base density of $\rho_0 = 1 \times 10^{-11}$ g cm$^{-3}$ and a $n$ of 2.4 \citep{marr2021}. CHECK VALUES

Finally, as previously shown, our three targets also have $n < 3.5$: $n = $ for \bcmi, $X$ for \acol, and $x$ for \aara. Looking further into this apparent trend, we turned to the survey of \citet{klement2019} on SED turndown in Be stars. In their Table 7, the authors compile the found values for $n$ for the Be stars in their sample that can be considered stable, and that show clear signs of SED turndown. We crossmatch their results with the values found for the same stars in \citet{vieira2017}'s survey, finding 12 stars that were a target in both works, and compare the values of $n$ derived in Table \ref{tab:robvsrod} and Fig \ref{fig:nvsn}.


\begin{table*}
    \centering
    \begin{tabular}{c|ccc|ccc}
    \hline
        \multicolumn{1}{c}{\textbf{Star}} & \multicolumn{3}{c}{\citet{vieira2017}} & \multicolumn{3}{c}{\citet{klement2019}}\\
        \hline
        % &  & Rodrigo& & Klement \\
        HD & $n$ (AKARI) & $n$ (WISE) & Mean $n$ & $n$ (IR) & $n$ (Radio) & Mean $n$  \\
        \hline
        5394  & 3.29 & - & 3.29 & 2.92 & 2.96 & 2.94\\
        23630  & 2.9 & 3.2 & 3.05 & 2.89 & 3.02 & 2.95\\
        25940  & 2.8 & 2.7 & 2.75& 2.46 & - & 2.46\\
        32343  & 2.2 & 2.0 & 2.1 & 2.06 & - & 2.06\\
        \textbf{37795}  & 2.5 & 2.5 & 2.5 & 2.69 & - & 2.69 \\
        41335 & - & 3.0 & 3.0 & 2.85 & - & 2.85 \\
        \textbf{58715}  & 3.0 & 2.7 & 2.85 & 3.13 & 3.44 & 3.285\\
        91465  & 3.1 & 3.3 & 3.2 & 2.65 & - & 2.65\\
        105435  & 2.8 & 3.0 & 2.9 & 2.44 & - & 2.44\\
        109387  & 2.5 & 2.6 & 2.55 & 2.78 & - &2.78\\
        148184  & 2.9 & 3.1 & 3.0 & 2.58 & - & 2.58\\
        \textbf{158427}  & - & 2.9 & 2.9 & 3.16 & - & 3.16\\
        \hline
    \end{tabular}
    \caption{ Crossmatch of stable Be star radial density exponent derived by \citet{vieira2017} and \citet{klement2019}. The bold stars are \acol, \bcmi and \aara.}
    \label{tab:robvsrod}
\end{table*}


\begin{figure}
    \centering
    \includegraphics[scale=0.5]{fig/nhist.png}
    \caption{\footnotesize Histogram of the values of $n$ from \citet{vieira2017} (in purple) and \citet{klement2019} (in orange)}
    \label{fig:nhist}
\end{figure}

For the stable CBe stars sampled in both surveys, all 12 show a $n < 3.5$ consistently in both studies (Fig. \ref{fig:nvsn} and histogram in Fig. \ref{fig:nhist}). We also did a quick study of the $n \sim 2.5$ CBe stars that are only in \citet{vieira2017}, searching for available \halp spectra on the BeSS database to check whether this stars appear to be stable. Out of 13 stars, we found 5 whose spectra do not change significantly over the period covered by the observations, but a more detailed analysis is needed confirm if they truly fall on this category.  


% 23552 - Espectro fica em 1.6, mudanças nos picos, largura parece n mudar mt

% 36576 - Muda bastante a altura e os picos tmb...

% 37697 - Altura muda (6 - 11), só um pico sempre

% 38010 - picos variam um pouco, mas parece bem estável

% 60606 - cRAZY

% 65875 - parece estável: um pico, altura muda um pouquinho (~10)

% 68980 - só 3 espectros, parece estável

% 86612 - EC muda bastante 

% 88661 - só 2 espectros, EC muda

% 109387 - muda d+, EC e picos

% 124367 - 1 espectro só

% 175869 - EC muda um pouco (+-0.2), picos tmb

% 185037 - parece estável, altura muda um pouquinho


\begin{figure}
    \centering
    \includegraphics[scale=0.7]{fig/nvsn.png}
    \caption{\footnotesize Comparing the mean values of $n$ derived by the surveys of \citet{vieira2017} and \citet{klement2019}.}
    \label{fig:nvsn}
\end{figure}

The fact that at least 14 stable Be stars (the 12 from the survey crossmatch plus $o$ Aqr and 66 Oph) have a radial density exponent confirmed to be smaller than 3.5 indicates that there is a factor missing in the power-law steady state solution of the VDD.

One possibility is that the disk is subject to thermal effects we are not considering in the steady state formulation when we assume an isothermal disk. This problem was studied by \citet{carciofi2008} by solving the non-isothermal viscous diffusion problem in the VDD formalism. The authors find that the effective slope of the disk,in this case, ranges between 2 and 3 for a radius $1 < r < 3$ $R_{eq}$, and between 3 and 3.5 for $r \leq 3 \, R_{eq}$. However, these strong effects are only seen for very dense discs. The possibility of a non-isothermal disk was investigated for the case of \bcmi, but found to be much too small to cause such changes in the structure of the disk, given its low density \citep{klement2015}. The denser disks of the other target stars could be affected by non-isothermal effects more strongly, leading to the observed effect on the density slope. Fig. \ref{fig:nvsrho} investigates if there is any significant correlation between $\rho_0$ and $n$ that could indicate non-isothermality in the disk. We find a weak positive correlation with a Pearson index of 0.39, once again the opposite of the behaviour expected if it were to explain the variation of $n$.

\begin{figure}
    \centering
    \includegraphics[scale=0.7]{fig/nvsrho.png}
    \caption{\footnotesize Comparison of the values of $n$ and log $\rho_0$ found by \citet{vieira2017} for all 14 stars in our sample.}
    \label{fig:nvsrho}
\end{figure}

It is also possible that the viscosity of the disk is variable with radius, which could lead to a less steep density fall-off. However, to date the only solid evidence of a radially varying viscosity was found in the Be stars: 28 CMa, but in that case it was \emph{growing} with radius, i.e., the reverse behaviour necessary to accommodate the $n$ results seen on our sample.  %From Eq. \ref{eq:VDDsigma}, we see that $\alpha$ and the temperature of the disk (which is part of $c_s$) have analogous effect on the density, so much that they can be considered a combined parameter $\alpha T$. However, when we consider the volume density $\rho \propto \Sigma/H$, the scale height $H$ has an individual dependence on the temperature, so a variable $T$ would influence the density differently. All in all, if either $\alpha$ or the temperature vary with the radius of the disk, their effect on its density structure could lead to an $n \leq 3.5$. However, this needs still to be further verified. Furthermore, 

Yet another possibility arises from the high incidence of SED turndown (see Sect. \ref{sec:disk_truncation}) and therefore binarity recently found among CBe stars. A consequence of binarity is the accumulation effect: an accumulation of matter in outer region of the disk due to the resonant torque caused by the companion. This pilfers some angular momentum from the disk, leading to a gentler, less steep fall-off of density as the radius increases (\citealt{okazaki2002}, \citealt{panoglou2016}). As all 14 stars from our sample shown signs of SED turndown or are confirmed binaries, this hypothesis is worth investigating.

The nature of the companions was not confirmed in \citet{klement2019} beyond the fact that they are invisible to the observables analysed, which indicates they are faint stars. It is also more likely that they are main sequence or sub dwarf stars, as cool G-, M-, or K- giant would dominate the spectra in the infrared region, what is not observed in the sample \citep{oudmaijer2010}. In \citet{panoglou2016}'s analysis, for their reference system with a primary with a mass of 11.2 $M_{\odot}$ and radius of 5.5 $R_{\odot}$ and binary mass ratio of $q = 0.08$, the torque of the companion is strong enough to lead to a measurable accumulation effect when the viscosity of the disk $\alpha$ $<$ 0.6, the orbital separation is $<$ 25 $R_{eq}$ and the period of the orbit is $<$ 55 days. As the mass ratio increases, the accumulation effect also becomes stronger. As such, in order to answer for the $n \leq 3.0$ trend we see in our sample, the CBe stars would need to have a close companion, in an orbit of less than a hundred days. The companion could be a sdO or sdB star, as their mass range of 0.40 - 0.55 $M_{\odot}$ \citep{zhang2010} culminates in mass ratios $0.02 < q < 0.19$ for the range of B stars masses. Perhaps the combined effects of accumulation of matter and non-isothermal viscous diffusion may be enough to explain the slope results. In either case, our findings pave the way for future developments on the VDD theory.


==> RESULTS_OLD.tex <==
\section{Results}\label{sec:results}
In this section we present the results of our MCMC implementation with \beatlas for our three targets: \bcmi, \acol and \aara. 
 
%Sect \ref{sec:results_sed_pol} shows the results obtained using SED and polarimetric data as inputs for our MCMC code. Results are compared to literature values in Sect. XXX. %Sect. XXXXX compares the synthetic \halp of the ``best'' model found for the targets with observed \halp. In Sect. XXX, we include \halp line profile as an input for the code, for the case of \acol.  

Each of the targets has a complete SED (from UV to radio) and a set of polarimetric data. As discussed in Sect. \ref{sec:targets}, all three stars can be considered as stable Be stars, as their observables imply that the disk has not undergone dissipation or any significant structural changes (such as $m = 1$ waves, which are common for Be stars) in the past decades. Therefore, their SED, although comprised of data gathered in different epochs, is considered here as a true snapshot of the emission of the Be star in a given moment. We also consider that the errors on any given measurement on the SED must be at least $10\%$ of the measured value, as the intrinsic variability of a Be disk over time, even for disks as stable as these, should be accounted for. The polarisation data used for the inference is an average of all measurements available for each of the 5 filters, and their errors are their median absolute deviation.



\begin{table}
%\centering
\small
\caption{Prior values for the targets. Parallax values are from Hipparcos \citep{vanleeuwen2007}; \vsini for \bcmi is from \citet{2015ApJS..217...29B}, \acol is from \citet{fremat2005}, and \aara from \citet{levenhagen2006}. \halp EW and FWHM values are derived from the collected data; no \halp EW and FWHM priors are used for \aara (see Sect. \ref{sec:methodology}).}
\label{tab:priors}
\begin{tabular}{l l l l l}
\hline\hline
Target & $\pi$ [mas] & \vsini [km/s] & \halp EW [\AA]  & \halp FWHM [km/s]\\
\hline
\bcmi & $20.17 \pm 0.20$ & $248 \pm 13$ & $-15.18 \pm 1.15$ & $299.81 \pm 5.88$\\
\acol & $12.48 \pm 0.36$ & $192 \pm 12$ &  $-29.15 \pm 2.80$ & $248.05 \pm 4.06$\\
\aara & $12.20 \pm 0.85$ & $270 \pm 25$ & - & - \\
\hline
\end{tabular}
\end{table}



\subsection{SED}\label{sec:results_sed}

We applied the method described in Sect. \ref{sec:methodology} for all available SED data of our targets. The values for all priors are given in Table \ref{tab:priors}. \ACR{SOBRE VSINI DE AARA: o bruno menciona 305+-15 na tese, mas não dá a referência, e não coloca na tabela 7.1 da tese tmb. estou usando o valor do Levenhagen, q cobre o valor do paper da catalina de 2018 tmb.} We opted for the Hipparcos determination of the targets' parallax over the more recent Gaia Data Release 3 (for \acol - the only target presented here that has a measurement) \citep{gaia2016} since it and Hipparcos disagree well above the nominal uncertainties, and Hipparcos' determination has a smaller uncertainty. Gaia also has several issues for bright and nearby sources which may have affected its determination of the targets' distances, and has known problems when dealing with binaries, which may the case for our targets as well.

All chains have 120 walkers. In order to assure convergence, simulations were run until the number of steps reached 50 times the autocorrelation time for all parameters, as recommended by \citet{Foreman-Mackey2013}, and until the autocorrelation time of all parameters changed less than 1$\%$ between subsequent estimates. 

To represent the PDFs using the standard ``value $\pm$ uncertainty'' notation, we chose to use the highest density region (HDR - also called highest probability region, or credible interval) of each PDF in $68\%$, with the mean value of this region as the ``best'' value for the parameter \citep{hyndman1996, chen2000}. The HDR does not have to be unique and continuous, but can be broken in more than one region, which allows us to explore multiple solutions that arise when the resulting distribution is not uni-modal. Thus, when a distribution is double-peaked, two sets of ``solutions'' are considered by us as physically possible results, and skewed distributions are better represented.


% \subsubsection{\bcmi}\label{sec:sed_bcmi}


Fig. \ref{fig:sed_corner_plot_bcmi} shows the result of the MCMC simulation for the complete SED of \bcmi, from 0.3 $\mu$m to 10 cm. The PDFs of all the parameters and their respective correlation maps are shown in Figure \ref{fig:sed_corner_plot_bcmi}). 


\begin{figure*}
\centering
\includegraphics[width=1.\linewidth]{figures/BCMI_FULLSED.png}
\caption{Corner plot for a MCMC simulation of \bcmi. See text for details. The inset shows the SED in the upper part and the residuals of the fit in the lower part. Black points represent observed data. The grey line is not a fit, but 300 random models of the sample that can be used as an estimate of the model uncertainties. Residuals of the fits of these random models are shown in the lower plot.}
\label{fig:bcmi_sed_corner}
\end{figure*}

The stellar parameters are well defined, specially the mass. The mass of a star is notably a difficult parameter to determine in general, and by far the best method for its determination is binary studies, in particular visual binaries for which all orbital elements can be determined. A 2$\%$ accuracy is the mass corresponds to a very good result in binary studies. The mass we determine in our modelling is more properly referred to as a ``theoretical'' mass, as it depends strongly on the underlying evolutionary model used in our methodology.

The rotation rate is in the range expected for Be stars. The disk has a relatively low density, and it is truncated at 33.65 \req. Being a galactic star, $E(B-V)$ is low. The prior on the distance constrains it to the Hipparcos determination quite closely.


% \subsubsection{\acol}\label{sect:sed_acol}

In Fig. \ref{fig:acol_sed_corner} we show the results for the simulation using the SED data for \acol. As explained in Sect. \ref{sect:metodology},
the likelihood function used in the MCMC sampling is a logarithmic $\chi^2$. However for \acol we have upper limit points in 2.0, 3.5 and 6.3 cm that are treated differently: the upper limits use a slightly modified version of $\chi^2$ in order to avoid discontinuities in the likelihood function (CADE ESSA REFERÊNCIAAAAAAAAAAAAAAAAA), as
%\begin{equation}
    %\chi^{2}_{\mathrm{uplim}} = - 2 \Sigma ( log( (pi/2.)^{0.5} rms (1. + %erf(((upper_lim - mod_upper)/((2^{0.5})*rms)))))) .
%\end{equation}

\begin{equation}
    \chi^{2}_{\mathrm{uplim}} = - 2 \, \Sigma \, \log\left[ \sqrt{\frac{\pi}{2}} \, \, \mathrm{rms}\left(1 + \erf{\left(\frac{\Delta}{\sqrt{2}*\mathrm{rms}}\right)}\right)\right],
\end{equation}\label{eq:like_chi2}

\noindent where
\begin{equation}
    \Delta = F_{\rm obs}^{\rm uplim} - F_{\rm mod}^{\rm uplim} .
\end{equation}

Thus, models which exceed the upper limits are greatly disfavoured by the sampler, and non-continuity(??) is avoided. 


\begin{figure*}
    \centering
    \includegraphics[width=1.\linewidth]{figures/acol_sed_corner.png}
    \caption{Same as Fig. \ref{fig:bcmi_sed_corner}, but for a MCMC simulation of \acol.}
    \label{fig:acol_sed_corner}
\end{figure*}

Similarly to \bcmi, our methodology provided impressive results, considering it only had the SED data to work with. The PDF for the radial density exponent $n$ is surprising: the expected value for an isothermal, steady-state VDD is $n = 3.5$. \citet{vieira2017} classified discs with $n \leq 3.0$ as dissipating discs. This is, however, inconsistent with what is know of \acol and \bcmi both, as their disks have been stable for decades. %\ACR{OLD - There is a second family of solutions shown in the corner plot of Fig. \ref{fig:acol_sed_corner}: a much smaller PDF centred on $\log n_0 \sim 11.95$ and in $n \sim 2.50$. This indicates that while the most likely solution is given by the densest region of the PDF, a less likely, but still possible solution exists and should not be completely discarded. Given that Be discs with $n \leq 2.0$ are very uncommon, and would be in active dissipation, our physical interpretation is that the second family of solutions ($n \sim 2.50$) is more realistic for \acol.}

The age \ttms derived indicates that \acol is at the end of its MS lifetime, and its rotation rate $W$ is within the expected range for a late-type Be star (REVISAR AQUI) \citep{rivinius2013}. As happened for \bcmi, the mass of the star is impressively well constrained, but again, this is an effect of the restrictions and inter-dependencies of the physical models behind \beatlas. The disk of \acol is also found to be truncated, with $R_D = xx$ \req, which may indicate the presence of a companion.

% \subsubsection{\aara}\label{sect:sed_aara}

Figure \ref{fig:sed_corner_plot_aara} shows the results obtained by considering the full SED. Like \acol, \aara also has upper limit points in the radio region, which are treated in the same manner, with the modified $\chi^2$ likelihood (Eq. \ref{eq:like_chi2}). 

Notably, the code has difficulty in fitting the lower UV spectrum, as shown by the residuals in the inset of Fig. \ref{fig:sed_corner_plot_aara}. This results in broader PDFs for all parameters.

\begin{figure*}
\centering
\includegraphics[width=1.\linewidth]{figures/aara_SED.png}
\caption{Corner plot for a MCMC simulation of \aara. See text for details. The inset shows the SED in the upper part and the residuals of the fit in the lower part. Black points represent observed data. The grey line is not a fit, but 300 random models of the sample that can be used as an estimate of the model uncertainties.}
\label{fig:sed_corner_plot_aara}
\end{figure*}

\aara's status as a B2 star is confirmed in our results, which give it a much higher mass than for either late-types \bcmi or \acol. Furthermore, its rotation rate is XX, lower than \bcmi's and \acol's. This highlights the known dependency of $W$ with temperature (and thus stellar type) of Be stars (\citealt{cranmer1996}, \citealt{huang2010}), where $W$ is generally lower (although still significantly large, as per Be stars classical characteristics) for high mass B stars than for lower mass. 

Once again sign of disk truncation is present. Considering our only criteria for selecting these three targets was their relative stability and brightness, the fact that all three of them are truncated lends some strength to the recurring idea that Be stars are the by-products of mass transfer binary systems.

CAN I MENTION ROBERT'S DETECTION OF THE COMPANION?? leave this to the discussion?

\subsection{Correlations}

\ACR{Isso fica nos resultados ou na discussão?}

The correlations between each couple of parameters are shown in the maps in the corner plots of Figs. \ref{fig:sed_corner_plot_bcmi}, X AND X. The corresponding correlation map for each of the pairs of parameters is plotted where they intersect in column and line. The behaviour of the correlations between the different parameters is very similar for all three targets, even though the targets are very different, as \aara is a late-type B star and \acol and \bcmi are early types.

Out of all the parameters explored, the extinction $E(B-V)$ has the most significant correlations with nearly all parameters. The cause is likely the interdependence of the parameters. Its connection with the mass is clear: the $E(B-V)$, as well as the mass, strongly affects the UV domain. The stronger the extinction, the less UV flux reaches the observer. As such, it would be necessary to have a more massive star to reach the same amount of flux as a less massive star seen with a smaller $E(B-V)$. Similarly, $W$ and $i$ both affect the stellar flux output in the UV, given the oblateness of the central star and the gravity darkening effect, and are themselves clearly intercorrelated. With such strong correlations with the stellar parameters, its connections are propagated, leading to second-degree correlations with disk parameters $n_0$, $n$ and $R_D$.

Flux excess in the IR is caused by reprocessing and re-emission of stellar flux by the disk. Therefore, the amount of excess is varies with the disk density, but also depends on the stellar parameters, which explains the correlations of mass, $W$ and age with $n_0$, $n$ and $R_D$. The concept of pseudo-photosphere of \citealt{vieira2015} is useful to explain the correlations among the three disk parameters. In this model, the disk emission can be approximated as the sum of two disk components: an inner region, optically thick pseudo-photosphere and an outer region, optically thin. The larger the emitting area of the pseudo-photosphere, the less energetic the flux emitted. The disk radius, base density and radial density exponent all control, in different ways, the size of the pseudo-photosphere, therefore leading to their interconnected correlations.

The correlations of the inclination angle of the system with $W$, $n$, $R_D$ and $n_0$ are due to the asymmetric nature of Be star. The central star is oblate, and therefore the inclination affects how its rotation is perceived. There is also the disk, which will have a smaller emitting area depending on the inclination angle at which we see the system. The high rotation also leads to differences in the temperature between the poles and equator of the star. A Be star seen pole-on will be perceived as hotter and brighter than a Be seen edge-on, even if there was no disk present.

The mass, rotation rate and time of life on the MS, \ttms, are also intercorrelated. In the \beatlas grid, $W$ and \ttms are theoretical parameters derived from $M_{\star}$ $R_{\rm pole}$ and luminosity, the physical parameters the \hdust radiative transfer code uses in its calculations. This then makes the parameters interdependent, in particular $W$ and \ttms, both of which strongly affect the physical size of the Be star either by the oblateness or by the inflation resulting from stellar evolution along the MS.

Finally, the distance affects the overall flux that reaches the observer, correlating strongly with the mass of the star and the three disk parameters, that have the greatest control over the flux in various wavelengths.

Deriving the correlations of the parameters along with their PDFs was an important factor in our early choice for employing Bayesian-MCMC techniques in our work with \beatlas. As such, this is the first study of Be stars that is able to obtain and quantify the correlations of its parameters, both stellar with stellar, disk with disk, and stellar and disk self-consistently. 



\subsection{Modelling Different Sections of the SED}

The concept of pseudo-photosphere suggests another approach to study the target. As seen in Fig. 13 of \cite{vieira2015}, the size of the pseudo-photosphere relates to the wavelength of the emission, with larger areas being responsible for the emission in larger wavelengths \citep{carciofi2011}. To investigate how much information each section of the SED carries about different model parameter, we split the SED in different sections and performed MCMC simulations in each, and for several combinations of these sections. The results are displayed in the violin plots of Fig. \ref{fig:violinplots}. The abscissa indicates the SED section used. Each plot corresponds to a given parameter, as indicated. For instance, the upper plot in the first column represents the inference of the stellar mass for each spectral domain analysed. In general, we verify that shorter wavelengths (UV, visible and near-IR) are more successful in constraining the stellar parameters: $M$, $W$, and \ttms. On the other hand, the disk parameters (mainly $R_\mathrm{D}$) are poorly constrained by these spectral domains. When we include the mid-IR domain is a global improvement of the inference is seen, especially in the disk parameters, $\log n_0$, $R_\mathrm{D}$ and $n$. The stellar parameters are much worse constrained when we remove the short wavelengths from the analysis. Overall, the best results were obtained when the full SED was used. This is easily understood by the strong correlation seen among most of the parameters: the removal of part of the data may result in a worse determination of one or more parameters that propagates to all others.


\begin{figure*}
\centering
\includegraphics[width=.8\linewidth]{figures/Violinplots_bcmi.png}
\caption{Violin plots of the PDFs of different spectral domains for all parameters of our three targets: blue violins for \bcmi, green for \acol, and red for \aara. The abscissa indicates the SED section used.}
\label{fig:violinplots}
\end{figure*}



% ........................................................................................................................................
\subsection{Polarisation}

The linear polarisation is strongly dependent on the number of scatterers (free electrons) and their geometry. Because the disk density, and hence the number of scatterers, drops quickly with radius, the bulk of the polarised light is created close to the star (see Fig. 1 of \citealt{carciofi2011}). Therefore, the most relevant parameter related to the amount of light that is polarised is the density at the base of the disk,$n_0$, rather than its size and radial exponent. The polarisation also depends strongly on the angle between the plane of the disk and our line of sight, so we also expect this observable to provide constrains to the inclination angle (\citealt{haubois2014}; \citealt{halonen2013}). 

As it is scattered light, the polarisation also heavily hinges on the central star parameters. The number of scatterers in a Be disk is given by

\begin{equation}
N_\mathrm{e} = 2\pi \int_{R_{\mathrm{eq}}}^{R_\mathrm{D}} r \Sigma(r)dr = f(R_{\mathrm{eq}}, n, n_0, R_0),
\end{equation}

\noindent and therefore, $N_\mathrm{e}$ depends on the radius of the star. But polarisation alone cannot provide strong constraints on the stellar properties, being generally blind to them. Since all parameters are strongly correlated, this blindness makes it impossible for the code to correctly make any determinations regarding the disk parameters too, even the ones polarimetry is privy to. To remedy this, we set additional priors for the MCMC polarisation simulation, based on the previous results obtained for the stellar parameters from the entire SED. We adopt a Gaussian kernel density estimator KDE\footnote{\url{https://jakevdp.github.io/blog/2013/12/01/kernel-density-estimation/}.} for the PDF of each stellar parameter ($M$, $W$ and $t/t_\mathrm{MS}$) constrained previously. This additional prior function becomes,

\begin{equation}
\log p_\mathrm{\star}(\Theta,\alpha) = -0.5 \, \left[\hat{f}_\mathrm{M}(M) + \hat{f}_\mathrm{W}(W) + \hat{f}_\mathrm{t/t_\mathrm{MS}}({t/t_\mathrm{MS}}) \right]^2,
\label{eq:prior_star}
\end{equation}

\noindent where $\hat{f}_\mathrm{M}$,  $\hat{f}_\mathrm{W}$ and $\hat{f}_\mathrm{t/t_\mathrm{MS}}$ are the inverse of the KDE distributions.


% \subsubsection{\bcmi}\label{sect:pol_bcmi}
Using the above priors, the result of the MCMC simulation for \bcmi (Fig. \ref{fig:kde_corner_plot_bcmi}), \acol (Fig. X) and \aara (Fig. X). Using the KDE priors of the stellar parameters allowed for inferring the disk base density and the inclination, as expected from the physical nature of polarisation. Most importantly, the values of these parameters agree with the previous determination shown in Fig. \ref{fig:sed_corner_plot_bcmi}. This is relevant because these two independent observations (SED and polarisation) probe different disk regions and are due to different physical processes in the disk (free-bound and free emission vs. polarisation).

To find a set of PDFs that take into account the information found by full SED (Fig. \ref{fig:sed_corner_plot_bcmi}) and polarisation (Fig. \ref{fig:kde_corner_plot_bcmi}) individual simulations, we multiply the two results, obtaining the corner plot shown in Fig. \ref{fig:comb_corner_plot_bcmi}.

% The results are shown in Table \ref{tab:best_params_bcmi} and are referred to in the following text as our ``best-fit'' values and their uncertainties. 

\begin{figure*}
    \centering
    \includegraphics[width=1.\linewidth]{figures/POLtruemedian_HDR.png}
    \caption{\beatlas simulation of \bcmi polarisation data using the \texttt{KDE} priors on the stellar parameters (see text).}
    \label{fig:kde_corner_plot_bcmi}
\end{figure*}



% % Routine: print_table_results.py
% \begin{table}
% \centering
% \caption{TO BE REVIEWED Best fit parameters of $\beta$ CMi. Free parameters: $M$, $W$, $t/t_\mathrm{MS}$, $\log \, n_0$, $R_\mathrm{D}$, $n$, $i$, $d$, $E(B-V)$. Derived parameters: $\log g$, $R_\mathrm{pole}$, $L$, $T_\mathrm{eff}$, $\beta_\mathrm{GD}$. }
% \label{tab:best_params_bcmi}
% \begin{tabular}{ll|ll}
% \hline\hline
% Parameter                              & Value                              & Parameter                           & Value                       \\ \hline

% $M\, [\mathrm{M_\odot}]$               & $4.13_{-0.15}^{+0.15}$             & $\log \, n_0$                       & $11.96_{-0.11}^{+0.18}$     \\

% $\log g$                               & $4.047_{-0.001}^{+0.001}$          & $R_\mathrm{D}\, [\mathrm{R_\star}]$ & $35.30_{-11.35}^{+9.96}$    \\
% $R_\mathrm{pole}\, [\mathrm{R_\odot}]$ & $3.20_{-0.03}^{+0.04}$             & $n$                                 & $2.43_{-0.18}^{+0.25}$      \\
% $L\, [\mathrm{L_\odot]}$               & $365.3_{-28.2}^{+31.2}$            & $i$ $[\mathrm{^o}]$                 & $42.19_{-2.19}^{+5.89}$     \\
% $T_\mathrm{eff}\,[\mathrm{K}]$         & $14080.88_{-215.24}^{203.04}$      & $d\, [\mathrm{pc}]$                 & $49.95_{-0.40}^{+0.43}$        \\
% $W$                                    & ${0.82}_{-0.04}^{+0.05}$           & $\beta_\mathrm{GD}$                 & $0.21_{-0.04}^{+0.04}$      \\
% $t/t_\mathrm{MS}$                      & $0.64_{-0.09}^{+0.09}$             & $E(B-V)\, \mathrm{[mag]}$           & $0.03_{-0.01}^{+0.01}$      \\ \hline
% \end{tabular}
% \end{table}


% \subsubsection{\acol}\label{sect:pol_acol}

%The lack of variability of the polarisation level of \acol, shown in Sect. %XX, is a strong indication of its stable disk. 
% As done for \bcmi, we ran our code using the polarisation as input and the results for the three stellar parameters obtained from the SED simulation as KDE priors. 

% Following the same procedure, the results for \acol and \aara are quite similar. 

% As expected given the nature of polarisation, the base density $\log n_0$ is well defined, and it coincides with the result obtained by the SED simulation. The inclination also matches within the errors, and the difference likely is due to the fact that the $v\sin(i)$, the prior that allows us to constrain the inclination in the SED simulation, is measured from He I and Mg II lines, a completely separate observable from polarisation.

% \subsubsection{\aara}\label{sect:pol_aara}











==> TARGETS.tex <==
% SECTION 4
% ========================================================================================================================================



\section{Targets' Overview}\label{sec:targets}

Three Be stars were selected as test cases for our method: the late-types \bcmi, which was the target of a very in-depth characterisation by \citet{klement2015}, and \acol, and the early-type \aara. All targets are known for having very little stellar and disk variability, and therefore are a good match for the VDD steady-state approximation \beatlas uses. Here we present a summary of the observational data collected for each target.


\subsection{\bcmi}\label{sect:overview_bcmi}

\bcmi (HD58715, HR2845) is a late-type (B8V) Be star, located inside the local bubble, about 50 pc away \citep{vanleeuwen2007}. \bcmi was the target of pioneer interferometric studies. For instance, \citealp{1997ApJ...479..477Q} published the disk and stellar diameters from interferometric measurements. They also estimated the equatorial radius, $R_\mathrm{eq} = 3.6 \, \mathrm{R_\odot}$, and a lower limit for the disk size, $R_\mathrm{D} = 13 \, \mathrm{R_\odot}$. Later, \citealp{2005ApJ...624..359T}, also through long-baseline interferometric data, determined the rotation rate ($W = 0.85 \pm 0.21$) and the equatorial radius, $R_\mathrm{eq} =  3.6 \pm 0.3 \, \mathrm{R_\odot}$, obtained from H$\alpha$ channels. \bcmi is one of the rare cases of a Be with a disk that has been stable for many years: it has been extensively observed in the past few decades, and no significant variation has been detected in either spectral lines or polarisation.

Recently, \bcmi was the target of the multi-technique analysis of \citealt{klement2015, klement2017}. \citealt{klement2015} represents a landmark in the Be literature, as it is still the most comprehensive model of a Be star to date. Table \ref{tab:bcmi_parameters} shows the best-fit parameters of each study. One interesting result was the detection of a SED turndown, a steepening in the slope of the SED in the radio, that was successfully modelled by a truncated disk (see Table \ref{tab:bcmi_parameters}). Under the assumption that the truncation was due to an orbiting companion, the authors used the results of \cite{panoglou2016} to predict the semi-major axis and the orbital period of the secondary, which was later found by \cite{dulaney2017} by means of radial velocity (RV) measurements. The detection was, however, questioned by \citet{harmanec2019}, who noted that the RV signal was perhaps contaminated. \citet{wang2018} also found no sign of a sdOB secondary when analysing \bcmi's UV data.

Most of the observations used here are the same as the ones used by \cite{klement2015}, but not all. We combined data from the literature, including photometric, polarimetric and spectroscopic data. Most data were accessed through online Virtual Observatory Tools (VO): \href{http://basebe.obspm.fr}{BeSS}\footnote{\url{http://basebe.obspm.fr};}, VO SED Analyzer (VOSA, \citealt{2008yCat..34920277B}), Spectral Analysis Tool (VOspec; \citealt{2008ASPC..394..227A}), \href{http://archive.stsci.edu}{MAST}\footnote{\url{http://archive.stsci.edu};}, \href{http://vao.stsci.edu}{VAO}\footnote{\url{http://vao.stsci.edu};}, \href{http://www.sdss.org}{SDSS}\footnote{\url{http://www.sdss.org};}, \href{http://www.aavso.org}{AAVSO}\footnote{\url{http://www.aavso.org};},  \href{http://archive.eso.org}{ESO archive}\footnote{\url{http://archive.eso.org};}, \href{http://vao.stsci.edu}{US Virtual Astronomical Observatory}\footnote{\url{http://vao.stsci.edu};}, and from VizieR Photometry viewer \citep{2000A&AS..143...23O}. The high resolution (R = 48000) \halp profiles used for this work are from ESO's FEROS, on the 2.2m telescope at the La Silla.

% ........................................................................................................................................
% \subsubsection{Photometric and UV Data}\label{sect:photometric_data}

The photometric data comprises results of several observers and missions: \cite{2002yCat.2237....0D}, Hipparcos \citep{1997yCat.1239....0E}, \cite{1994yCat.2193....0M}, 2MASS, TYCHO \citep{2000yCat.1259....0H} in the visual domain, DENIS, IRAS, WISE \citep{2014yCat.2328....0C} in the IR domain, AKARI (AKARI/IRC mid-IR all-sky Survey; \citealt{2010A&A...514A...1I}), MSX (MSX6C Infrared Point Source Catalog; \citealt{2003yCat.5114....0E}), SDSS, and from the Catalogue of Homogeneous Means in the UBV System \citep{1994yCat.2193....0M}. UV data from the International Ultraviolet Explorer (IUE)\footnote{\url{http://sci.esa.int/iue/31284-summary/}}, obtained from the \href{INES Archive Data Center}{http://sdc.cab.inta-csic.es/cgi-ines/IUEdbsMY}\footnote{\url{http://sdc.cab.inta-csic.es/cgi-ines/IUEdbsMY}} was used. Only high-dispersion large-aperture observations were selected for all our targets, as they can be flux calibrated.


\cite{klement2015} modelled \bcmi up to the radio region, using data from APEX/LABOCA, as well as VLA, and data from the literature. In the 2017 revision of the model \citep{klement2017}, new VLA data was made available. Recently, the authors obtained the first 5 cm and 10 cm measurements of a Be disc, and these were kindly made available to us. The radio data is summarised in Table \ref{tab:radio_data_bcmi}.

\begin{table}
\caption{Recent radio data of \bcmi.}
\label{tab:radio_data_bcmi}
\centering
\begin{tabular}{l l l l l}
\hline\hline
Band & $\lambda$ & Flux        & Flux Error       & Reference               \\
     & [cm]         & $[\mathrm{erg/s/cm^2/\AA}]$ & $[\mathrm{erg/s/cm^2/\AA}]$ &                        \\ \hline
K    & 1.36       & 2.24 $\times 10^{-24}$    & 2.76 $\times 10^{-25}$    & R. Klement, priv. comm. \\
X    & 3          & 1.56 $\times 10^{-25}$    & 1.33 $\times 10^{-26}$    & R. Klement, priv. comm. \\
C    & 5          & 2.90 $\times 10^{-26}$    & 2.64 $\times 10^{-27}$    & R. Klement, priv. comm. \\
S    & 10         & 2.28 $\times 10^{-27}$    & 6.00 $\times 10^{-28}$    & R. Klement, priv. comm. \\
     & 0.087      & 1.53 $\times 10^{-20}$    & 1.23 $\times 10^{-21}$    & APEX/LABOCA   \\ \hline          
\end{tabular}
\end{table}

% ........................................................................................................................................
% \subsubsection{Linear polarisation Data}\label{sect:linear_polarisation}
We made use of polarimetric data from the Pico dos Dias Observatory (OPD-LNA) (Tab. \ref{tab:polarimetric_bcmi_data}), and from the HPOL Spectropolarimeter at the University of Wisconsin-Madison Pine Bluff Observatory (PBO) \href{https://archive.stsci.edu/hpol/}, obtained from the {\texttt{MAST} Archive}\footnote{\url{https://archive.stsci.edu/hpol/.}}(Tab. \ref{tab:specpol_bcmi_data}). 



\subsection{\acol}\label{sect:overview_acol}

\acol (HD37795, HR1956) is a late-type Be star (listed as B9Ve, \citealt{levenhagen2006}) of the Southern hemisphere. Being a bright star ($m_v$ = 2.65), it has been the target of many observations over the years. Since its discovery as a Be star in 1897 \citep{jaschek1964}, \acol showed very little variation, as noted by \citet{jaschek1964} in their spectroscopic survey. \citet{dachs1981} and \citet{slettebak1982} also detected no major variation in their observations of the star, and it has never been reported to have gone on an inactive phase. Thus, \acol, like \bcmi, can be considered a stable Be star, and its long observational history make it a good candidate for this work.

For the UV region of the spectrum, we used data from  obtained from the INES Archive Data Centre, as was for \bcmi. Further SED data was collected from VOSA, from the catalogues Hipparcos \citep{esa1997}, 2MASS \citep{2mass2006}, TYCHO \citep{hog2000}, and the Catalogue of Homogeneous Means in the UBV System \citep{mermilliod1997} in the visual, and IRAS\footnote{\url{https://irsa.ipac.caltech.edu/Missions/iras.html}}, WISE \citep{cutri2014} and AKARI \citep{doi2015} in IR. We also have an APEX measurement from the European Southern Observatory's LABOCA instrument at $870 \: \mu$m \citep{klement2017}, and literature upper limit data from \cite{clark1998} (Australian Telescope Compact Array - ATCA) and \cite{taylor1990} (National Radio Astronomy Observatory's Very Large Array - VLA) in the radio region, at 2, 3.5, and 6.3 cm.

%We selected the spectra taken in IUE's large aperture mode, comprised of a oval window of 10x20 arcsec, as there was only one spectra available with the small aperture configuration. 13 spectra were obtained in total, 3 with the Long Wavelength Prime camera (covering from 1850 to 3350\AA) and 10 with the Short Wavelength Prime camera (1150-1980\AA). There was only high dispersion data available. There was no significant variation in the spectra, therefore they are simply averaged and binned for the modelling procedure.


\begin{figure*}
    \centering
    \includegraphics[scale=1]{figures/FINAL_ACOL.pdf}
    \caption{Polarisation, \halp line measurements and metals lines profiles for \acol. Upper panel: equivalent width (EW), emission over continuum (EC), peak separation (PS) and violet over red variation (V/R) for \halp (profiles in right uppermost panel).
    Lower panel: OPD polarisation data for B, V, R and I filters, by date of observation. The shaded region indicates $\pm 1 \sigma$ from the mean value of the data for each filter.
    Right panel: all profiles for \halp, He I 6678, He I 5877, He I 4713, He I 4473, He I 4388, Fe II 5317, Fe II 5169; overplotted in black is the mean spectrum.}
    \label{fig:overview_acol}
\end{figure*}

The polarimetric data used in this project comes from the Pico dos Dias Observatory (OPD) in Minas Gerais, Brazil. The data for U, B, V, R and I filters are shown in Fig. \ref{fig:poldata}. It is clear that variation is minimal, mostly contained withing 1$\sigma$ of the mean value, indicated by the yellow region. This result confirms that $\alpha$ Col is not in a process of disk build-up or dissipation, both of which would be noticeable in polarisation data. If further indicates that the mass injection rate into the disk is very steady over time.


For \acol, \halp line profile data was also collected for this work, as it provides insight into the general stability of the disk, an important factor to consider when using our method. As \bcmi was already previously studied in detail in this front by \citet{klement2015}, we point to this work for further spectroscopic analysis of this target.

There were available \halp spectra from the BeSS\footnote{\url{http://basebe.obspm.fr/basebe/}} and BESOS\footnote{\url{http://besos.ifa.uv.cl}} catalogues, as well as FEROS (from Th. Rivinius and N. Leister), UVES (from ESO's Science Portal\footnote{\url{http://archive.eso.org/scienceportal/}}), ESPaDOnS\footnote{\url{http://www.cadc-ccda.hia-iha.nrc-cnrc.gc.ca/AdvancedSearch/}} and NRES\footnote{\url{https://lco.global/observatory/instruments/nres/}} data. There were also data obtained at OPD using both ECASS and MUSICOS spectrographs. 

As they were collected from different sources, each batch of spectra has different resolution and calibration in general. ESPaDOnS is a fibre-fed high-resolution echelle spectrograph on the Canadian-France-Hawaiian Telescope (CFHT) reaches an average spectral resolution of about 70000. The BeSS spectra come from various sources: all spectra were taken with a Lhires III spectrographs, but mounted on different telescopes (4 on a Celestron 11, 1 on a RC14 and 1 on a Celestron 8), and all have a mean resolution of 14000. BeSOS spectra are taken with a high resolution echelle spectrograph called PUCHEROS, with a resolution of 17000. OPD data are taken with either the MUSICOS fibre-fed high-resolution echelle spectrograph, with a resolution of 35000, or with ECASS, a low-resolution (4000) Cassegrain spectrograph. ESO's FEROS is a very high-res echelle spectrograph, with R = 48000, while UVES is a high-res optical spectrograph, able to reach R = 75000. NRES spectrographs have a resolution of R = 53000. 

Be star disks, being formed by material ejected from the central star, are subject to variability in many time scales. As \halp is formed in a large area in the disk, its variability is connected with dynamics occurring in the disk. Double peaked profiles in emission lines caused by the Doppler effect of the disk's rotation are characteristic of this type of star when viewed in intermediate inclinations. Thus, several quantities are interesting for \halp analysis in Be stars: peak separation ($PS$), defined as the distance, in $\mathrm{km\,s^{-1}}$, between the red and violet peaks; equivalent width ($EW$), defined as

\begin{equation}
        EW = \int \left(1 - \frac{F_\mathrm{\lambda}}{F_0}\right) \,d\lambda \, ,
\end{equation}
    
where, $F_0$ represents the continuum and $F_\lambda$ represents the intensity across the wavelength range of interest; emission over the continuum ratio ($E/C$), which is the ratio between the highest value of the emission profile over the adjacent continuum; and finally the $V/R$, the relative strengths of the two peaks (violet on red, or V/R variations), which can indicate variability in the disk structure. We plot this quantities for \acol in Fig. \ref{fig:overview_acol}. 

\ACR{eu gosto desse texto, mas n sei se aqui é o melhor lugar para ele...}
Even if a Be star is itself stable, with no explosive mass ejection episodes, it is still possible to arouse variation in the disk by other, external means. A binary companion in a close orbit, for instance, has been proven to be able to excite two armed (m=2) density waves in the disk and to truncate the disk as the resonant torque it exerts on the Be disk prevents it from growing past the companion's orbit (\citealt{okazaki2002}, \citealt{panoglou2016}). If intense enough, the two armed density waves leave a clear observational counterpart in the emission lines: as they travel through the disk following the orbital motion of the companion, the density is increase in one or other side of the disk cyclically. This leads to an increase in the emission of the red and violet peaks of the emission line in turns. The periodicity of the V/R variation in binary Be stars can in some cases have the exact same period as the orbital period of the system, as is the case for $\pi$ Aqr \citep{zharikov2013}.

Periodic radial velocity shifts can also be indicative of the presence of a binary companion. The strong emission in \halp makes it the best target to look for such signals, as other lines are too broadened by the rotation of the star. Although our dataset contains a significant amount of observations, many are from the same or consecutive nights, which did not allow us to detect any type of signal, either in V/R or RV that this star has a binary companion.  

Metallic lines, on the other hand, form either on the photosphere of the star or on its innermost disk, not so strongly affected by a companion or other external factors. So, they are sensitive to changes arising from the central star. Be stars are, as a class, pulsators, as proven by recent works with space photometry (citar os paper do dietrich e o do jon e do rivi tmb). Signs of a Be star's pulsational modes can sometimes as periodic line profile variability in their metal lines, such as HeI, FeII, MgII and SiIII \citep{rivinius2003}. Fig. \ref{fig:overview_acol} shows that small scale variability is indeed present in \acol for HeI and FeII which may be connected to pulsational signals. Unfortunately, no counterpart was found in space photometry of \acol from the TESS mission, which displays only periods related to stellar rotation \citet{balona2020}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AARA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\aara}\label{sect:overview_aara}
The southern star \aara (HD 158427, HR 6510) is a MS star of spectral type B2Vne according to \cite{2006MNRAS.371..252L}.%; however, it is a good example of a star that has been classified very differently in the literature (see below). 
Its proximity ($74.3 \, \mathrm{pc}$, \citealt{2007A&A...474..653V}) and brightness (V = 2.93) allowed for the constitution of a rich observational dataset, offering unique opportunities to perform a detailed study of the process that governs the dynamic of Bes and their discs. The Arae region in the sky is suitable for such studies, given its lower extinction levels \citep{1980AJ.....85.1207V}.

\aara, like our other targets, has also shown a relatively stable behaviour over the years, in contrast with most early-type Be stars that have quite variable discs (\citealt{2018AJ....155...53L}; \citealt{2018MNRAS.476.3555R}). It has been the subject of several studies in the literature, targeting both the central star and its disk. %A summary of the results in the literature can be found in Tables \ref{tab:previous_models_aara} (stellar properties) and \ref{tab:previous_models_aara2} (disk properties). 
The stellar properties found in the literature vary widely (Tab. \ref{tab:previous_models_aara}: masses are reported in the range 6.2 - 9.5$\,\mathrm{M_\odot}$, and the polar radius varies by a factor of more than two (between 3.94 and 9.6), with corresponding discrepancies in the luminosity.

% Binarity/wind of alpha Arae
Possible binarity of \aara was first suggested from studies performed with the MIDI and AMBER interferometers \citep{2006EAS....18..273M}. The interpretation of these results, obtained using an outflowing disk model, suggested a dense polar wind along its rotational axis and a geometrically thin disk truncated by an unseen binary. These previous models suggested a period of $\sim \, 74 \, \mathrm{days}$ and a semi-major axis of 32 $R_\star$ for the companion ($M_\star \, < 2 \, \mathrm{M_\odot}$) (e.g. \citealt{2005A&A...435..275C}, \citealt{2007ASPC..361..518V}, \citealt{2007A&A...464...59M}).

Recently, \cite{2012A&A...538A.110M} concluded that the size of the emitting region does not differ in the range 8 - 12 $\mu \mathrm{m}$ from MIDI measurements (see Table \ref{tab:previous_models_aara2}). Their results are supported by \cite{2013JAsGe...2..125H}. These authors found that \aara's disk, between $2.1$ and $12 \, \mu \mathrm{m}$, does not change considerably and, according to them, this corroborates the hypothesis of a truncated disk by an unseen companion.

% Wind of Alpha Arae
About the suggestion that \aara has a dense polar wind, the recent review of \cite{2013A&ARv..21...69R} argues that the evidence proposed by \cite{2005A&A...435..275C} is weak, as it was based on a single interferometric measurement. Here, a simple calibration bias in the interferometric measurement could cause fluctuation in the derived size along the direction of the baseline of observations in the sky. Despite this, the interplay between winds and rotation should be better investigated. For instance, the combination of these effects could affect the stellar evolution and the mass injection to the circumstellar environment \citep{2013A&A...553A..24G}.

%\subsubsection{Photometric Data}\label{sect:photometric_data_aara}
The selection of the photometric data of \aara followed the same procedure described in Section \ref{sect:photometric_data}. The selected photometric data is in Table \ref{tab:photometric_data_aara}. Of particular importance for this project is the APEX/LABOCA measurement at $870\, \mu\mathrm{m}$. In addition to these, we found measurements at 3.5 and 6.3$\,\mathrm{m}$ by \cite{1998MNRAS.299.1119C}. Unfortunately these authors could not measure the flux, but still were able to set upper limits of $0.06$ and $0.2$ mJy, respectively. This new radio data gives us opportunity to investigate the claims of a binary companion reported above, using the SED turndown method employed for \bcmi (see Sect.~\ref{sect:results_bcmi}).

% Additional light curves were obtained from the tools \href{https://www.aavso.org/lcg}{AAVSO}\footnote{\url{https://www.aavso.org/lcg};}, \href{https://www.aavso.org/vsx/}{VSX}\footnote{\url{https://www.aavso.org/vsx/};} and from the Hipparcos mission (\href{http://vizier.cfa.harvard.edu/viz-bin/VizieR-3?-source=I/239/hip_main}{Hipparcos VizieR Table}\footnote{\url{http://vizier.cfa.harvard.edu/viz-bin/VizieR-3?-source=I/239/hip_main}.}).

% ........................................................................................................................................
%\subsubsection{Linear polarisation Data}\label{sect:linear_polarisation}


We made a complete search in the literature for published values of polarisation, summarized in Table \ref{tab:polarimetric_aara_data_2}. The observations made by our research group at OPD-LNA polarimeter and \cite{1979MNRAS.186..265M} are detailed in Table \ref{tab:polarimetric_aara_data}. One interesting feature of the data is the absence of large-scale variations in the polarisation.

\begin{table*}
\centering
\footnotesize
\caption{Full polarimetric dataset available for \aara. The table lists the average of all data and the standard deviation. Notes: $^\mathrm{a}$: Intrinsic values. $^\mathrm{b}$: The respective error is 0, according to \cite{2016MNRAS.455.1607C}. [1] \cite{2001A&A...368..912Y}. [2] \cite{2016MNRAS.455.1607C}. [3] \texttt{OPD-LNA}. [4] \cite{1979MNRAS.186..265M}.}
\label{tab:polarimetric_aara_data_2}
\begin{tabular}{l l l l l l l l}
\cline{4-4}
\hline\hline
MJD   & $P_{\mathrm{U}}$ [\%]  & $P_{\mathrm{B}}$ [\%] & $P_{\mathrm{V}}$ [\%]      & $P_{\mathrm{R}}$ [\%] & $P_{\mathrm{I}}$ [\%] & $PA_{\mathrm{int}}$ [$\mathrm{^o}$] & Ref.                             \\ \hline
-              & -                      & -                     & 0.58$^\mathrm{a}$          & -                     & -                     & $174^\mathrm{a}$                    & [1]  \\
56996          & -                      & -                     & $0.62400(34)$      & -                     & -                     & $172^\mathrm{b}$                    & [2]  \\
54260 to 57624 & $0.39 \pm 0.02$        & $0.61 \pm 0.05$       & $0.59 \pm 0.04$            & $0.48 \pm 0.01$       & $0.45 \pm 0.01$       & $142.2 \pm 2.6$                     & [3]                 \\
40085 to 42877 & $0.33 \pm 0.01$        & $0.67 \pm 0.01$       & $0.60 \pm 0.01$            & -                     & -                     & 172                                 & [4]  \\ \hline
\end{tabular}
\end{table*}


%\subsubsection{Stability}\label{sect:variability_aara}
The Be \aara was reported to be stable on long time-scales by \cite{1981A&AS...43..427D} and, in the words of \cite{1988A&A...189..147H}, ``still seems to represent an active Be star in a well-balanced equilibrium state". Its stability was reported by the study of $V/R$ variability and global oscillations by \cite{1995A&A...300..163H}, showing almost no variability in the line profiles over 7 years (see Fig. 12 in \citealt{1995A&A...300..163H}) and an equivalent width ($EW$, see below) of about 20-30 $\mathrm{\AA}$ over the same period. Earlier, \cite{1991A&A...241..159M} detected rapid $V/R$ variations from high time-resolution observations ($\sim 7$ days) between 1984 and 1989, having detected a quasi-period of $0.13 \, \mathrm{yr}$ ($\sim 47.5 \, \mathrm{days}$) using data from \cite{1988A&A...189..147H}. In another study, \cite{1991A&AS...88....1M} showed that \aara had a relatively constant and moderate H$\beta$ emission (see their Fig. 12) with $V/R$ variations of small amplitude, only slight changes in strength of emission and mean $EW$ relatively constant between 1977-87, except for a rapid decrease in 1982. In summary, these previous studies concluded that \aara might have had variations in timescales of months, however without showing a clear, organised long-term pattern. 

More recent \halp data was collected to analyse its current state. %A complete list of the \halp data of \aara is presented in \ref{add-data}. 
The spectroscopic data of \aara were gathered from VO tools, observatories and papers, in addition to new data taken at the OPD (ECASS and MUSICOS). We have data from Flash and Heros, covering from $3\,500 \, \mathrm{\AA}$ to $9\,000 \, \mathrm{\AA}$ (accessed with \href{http://dc.zah.uni-heidelberg.de/}{GAVO}\footnote{\url{http://dc.zah.uni-heidelberg.de/};}; ESO's UVES, FEROS, HARPS and CHIRES\footnote{CRyogenic high-resolution InfraRed Echelle Spectrograph} (providing high-resolution data from 1 to 5 $\mu$m \citealt{2004SPIE.5492.1218K}). Our compilation also includes historical digitalized hydrogen lines (H$\alpha$ and H$\beta$) published by \citet{1981A&AS...43..427D} (1978-11-02 to 1977-07-08), \citet{1996A&AS..116..309H} (1982-08-30 to 1993-09-09), \citet{2000A&AS..147..229B} (1999-04-13) and by \citet{1986A&AS...63...87D} (1982-02-27 to 1983-03-17).  

%     \item From the \texttt{ESO} facility\footnote{The reduction chain used for all instruments of the \texttt{ESO} followed the sequence: 1) classify/organise the data, a process called ``data association", which uses, in principle, \texttt{FITS} headers information present in ``association keywords". 2) Next, the instrument pipeline is called by a standard \texttt{ESO} application, i.e. \textsc{Gasgano} \citep{2012ascl.soft10020E}, \textsc{Reflex} or \textsc{Esorex} \citep{2013A&A...559A..96F};}, we obtained \texttt{UVES} data. This echelle spectrograph covers from $3\,000$-$5\,000 \, \mathrm{\AA}$ (blue arm) to $4\,200$-$11\,000 \, \mathrm{\AA}$ (red arm). Its spectral resolution can reaches up to $80 \, 000$ (blue arm) or $110\,000$ (red arm) \citep{2000SPIE.4008..534D}. We reduced the data using the \texttt{UVES} pipeline described in  \href{ftp://ftp.eso.org/pub/dfs/pipelines/uves/uves-pipeline-manual-22.12.pdf}{\texttt{UVES}-Tutorial}\footnote{\url{ftp://ftp.eso.org/pub/dfs/pipelines/uves/uves-pipeline-manual-22.12.pdf};}(version 5.7.0);

%     \item \texttt{CRIRES}\footnote{CRyogenic high-resolution InfraRed Echelle Spectrograph;} instrument provided high-resolution data from 1 to 5 $\mu$m \citep{2004SPIE.5492.1218K}. These data were reduced by the \textsc{EsoRex} platform \citep{2015ascl.soft04003E} as described in \href{https://www.eso.org/public/teles-instr/paranal-observatory/vlt/vlt-instr/crires/}{\texttt{CRIRES}-Tutorial}\footnote{\url{https://www.eso.org/public/teles-instr/paranal-observatory/vlt/vlt-instr/crires/}.} (see Tab. \ref{tab:spectroscopic_aara_data});
    
%     \item \texttt{Harps} and \texttt{Feros} reduced data were downloaded from \texttt{ESO} archive.
    
% \end{itemize}


Our collected polarisation and \halp spectra data are sumarized in Fig. \ref{fig:overview_aara}. The coloured band in each panel of Fig. \ref{fig:overview_aara} marks the median and the standard deviation of the mean. The properties of the \halp emission lines have remained roughly constant since 1978, in line with the results from the literature search reported above. However, the latest data (since 2012 or so) shows a deviation of this behaviour: one can see the $EW$ becomes larger (more negative), the $E/C$ ratio rises and the peak separation becomes smaller than the average value. One possible explanation for this behaviour is that the adjacent continuum of the line became suppressed, e.g., by a partial dissipation of the inner disc, thus causing both the $E/C$ and the absolute $EW$ to increase. Some hints indicating this partial dissipation of the inner disk may also be seen in Fig. \ref{fig:overview_aara}, mainly at the $B$ and $V$ bands.

\begin{figure*}
\centering
\includegraphics[width=1.\linewidth]{figures/FINAL_AARA.pdf}
\caption{Polarisation and \halp line measurements for \aara. Upper panel: equivalent width (EW), emission over continuum (EC), peak separation (PS) and violet over red variation (V/R) for \halp. Lower panel: OPD polarisation data for B, V, R and I filters, by date of observation. The shaded region indicates $\pm 1 \sigma$ from the mean value of the data for each filter.}
\label{fig:overview_aara}
\end{figure*}

% Variability: polarisation
To confirm the long-term and, more importantly, the \emph{recent} stability of \aara's disk, we plot in Fig. \ref{fig:overview_aara} the temporal evolution of the linear polarisation measurements (data from Table \ref{sect:obs_data_pol}). The red bands mark the median of the data and the width the standard deviation of the mean. The $BV$ data is spread over about 50 years, with a gap of $\approx 30$ years starting in 1976. Data for the $RI$ bands is available only since 2007. The polarisation levels are remarkably stable for all bands. More remarkable is the lack of variability between the seventies and the years 2000, which suggest that the disk has remained stable for 5 decades. As discussed above, several short-term variations were observed in the literature (e.g., the 1982 drop in the H$\beta$ emission seen by \citealt{1991A&AS...88....1M}). A similar feature is seen in the polarisation data. There is one drop in early 2007 (seen only in $B$ and $V$) and another, smaller one seen in early 2011 in all filters.





==> TESTING.tex <==

\\
\commentACC{mover o texto desta secao para as subsecoes correspondentes abaixo}
%\section{Target overview}\label{sect:targ_over}
\\

We introduce a novel method for estimating the parameters of Be stars using a comprehensive grid of radiative transfer models and an MCMC sampling algorithm. In order to critically test this method, we apply it to two well studied Be stars, \aeri and \bcmi, to certify that it can accurately recover the fundamental parameters of these stars. % \addACC{and to assess if the metodology allows 

\aeri ($\alpha$ Eridani, Achernar, HD10144, HR472, HIP7588) is the nearest Be star to Earth, at a distance of only $42.8 \pm 1.0$ pc ($23.39 \pm 0.57$ mas - \citealt{vanleeuwen2007}). It is well-known also for the drastic deformation it suffers due to its rapid rotation. Being such a close target, it has been the focus of several interferometric and imaging observations in the last decade. With PIONIER data, \citet{domiciano2014} imaged the photosphere of \aeri and measured its equatorial rotational velocity ($v_{\rm eq} = 298.8^{+6.9}_{-5.5}$
km/s), equatorial radius (\req $= 9.16 \pm 0.23 \, R_{\odot}$), inclination
($i = 60.6^{+7.1}_{-3.9} \degree$), and the gravity darkening exponent ($\beta_{\rm GD} = 0.166^{+0.012}_{-0.010}$). The discovery of its wide binary companion, \aeri B \citep{kervella2007} (with a period of $2570.94 \pm 0.53$ days, $\approx 7$ years), and the subsequent observations of \citet{kervella2022} allowed for a robust estimate of the mass of \aeri A, the Be star, as $5.99 \pm 0.60 M_{\odot}$.

The viscous disc of Be stars dissipates if matter stops being added to its base, i.e., if the mass ejection from the star ceases.
%\commentACC{cuidado aqui: o termo inactive é usado neste artigo \url{http://www.aanda.org/10.1051/0004-6361/201628411} -- ler primeiro parágrafo da secao 2 -- como sinonimo de estrela sem disco. Uma estrela ativa é a que tem disco.}
When this happens, the \textit{inactive} \citep{rivinius2016b} Be star is then perceived just as a fast rotating B star, as all its class-defining observational signals disappear. \aeri had recent inactive phases from 1970 to 1975 and in 2000, where no emission could be detected in its spectra, and phases of very weak emission between 1980 to 1990 \citep{vinicius2006} and after 2000. Therefore, data from these time periods are a good approximation for pure photospheric emission from \aeri. 

\bcmi ($\beta$ Canis Minoris, HD58715, HR2845, HIP36188), on the other hand, is one of the most stable Be stars known, having been active since its discovery \citep{merrill1925}, maintaining a stable disc with little variation. Also nearby \citep[$20.17 \pm 0.20$ mas,][]{vanleeuwen2007}, \bcmi was the target of several interferometric studies. \citet{1997ApJ...479..477Q} could estimate disc and stellar diameters such as the equatorial radius, \req $= 3.6 \, R_{\odot}$, and a lower limit for the disc size, $R_\mathrm{D} = 13 \, R_{\odot}$. Later, \citet{2005ApJ...624..359T}, also through long-baseline interferometric data, determined the rotation rate ($W = 0.85 \pm 0.21$) and found similar $R_\mathrm{eq} =  3.6 \pm 0.3 \, \mathrm{R_\odot}$. \bcmi is the first late-type Be star to show signs of non-radial pulsation \citep{saio2007}; spectrointerferometry and spectroscopy analysis of \bcmi provided important confirmation of the Keplerian nature of Be discs \citep{Wheelwright2012,Kraus2012}.

\bcmi was the target of the multi-technique analysis of \citet{klement2015, klement2017}. \citet{klement2015} represents a landmark in the Be literature, as it is still the most comprehensive model of a Be star to date
\citep[note that a corrigendum was published,][]{klement2015corrigendum}. One interesting result was the detection of a SED turndown, a steepening in the slope of the SED in the radio, that was successfully modelled by a truncated disk. \citet{dulaney2017} detected a companion in the system using radial velocity (RV) analysis, with a period of 170.4 days. The detection was, however, questioned by \citet{harmanec2019}, who noted that the RV signal might be contaminated. \citet{wang2018} also found no sign of a sdOB secondary when analysing \bcmi's UV data. Its status as a binary is therefore still not confirmed.

Given the nature of these two stars, we test our method using the photospheric \beatlas grid on the discless phases of \aeri, using International Ultraviolet Explorer (IUE) data (obtained from the INES Archive Data Center\footnote{\url{http://sdc.cab.inta-csic.es/cgi-ines/IUEdbsMY}}) from 1989 and a H$\alpha$ spectra from January 11th, 2000, taken with ESO's FEROS (high-res echelle spectrograph, $R$ = 48000), mounted at the 1.52m telescope in La Silla. 

We test the disc \beatlas on \bcmi using virtually the same data as \citet{klement2015}, which is summarized below. Photometric data were combined  from the literature using the Virtual Observatory VOSA \citep{2008yCat..34920277B}, comprising  results of several observers and missions: \cite{2002yCat.2237....0D}, Hipparcos \citep{1997yCat.1239....0E}, \cite{1994yCat.2193....0M}, 2MASS, TYCHO \citep{2000yCat.1259....0H} in the visual domain, DENIS, IRAS, WISE \citep{2014yCat.2328....0C} in the IR domain, AKARI \citep{2010A&A...514A...1I}, MSX \citep{2003yCat.5114....0E}, SDSS, and radio data from APEX/LABOCA and VLA. 
For the UV, data from IUE was used. For both \aeri and \bcmi, only high-dispersion large-aperture IUE observations were selected, as they can be flux calibrated. We also use polarimetric data taken from the Pico dos Dias Observatory. % \commentACC{como não reportamos novos dados, não vejo necessidade de repertir a tabela, pois é a mesma publicada pelo robert} (OPD-LNA - Tab. \ref{tab:polarimetric_bcmi_data})


%, and from the HPOL Spectropolarimeter at the University of Wisconsin-Madison Pine Bluff Observatory (PBO) \href{https://archive.stsci.edu/hpol/}, obtained from the {MAST Archive}\footnote{\url{https://archive.stsci.edu/hpol/.}}. 



% \begin{table}
% \centering
% \small
% \caption{Disk and stellar parameters of $\beta$ CMi obtained from the literature.}
% \label{tab:bcmi_parameters}
% \begin{tabular}{lll}
% \hline\hline
% Parameter & {\citealp{klement2015}} & {\citealp{klement2017}} \\ \hline
% $R_\mathrm{pole} [R_\odot]$                   & 2.8                                    & $2.8 \pm 0.2$                 \\
% $M \, [M_\odot]$                              & 3.5                                    & 3.5                           \\
% $L \, [L_\odot]$                              & 185                                    & $185 \pm 5$                   \\
% $W$                                           & 0.98                                   & 1.0                           \\
% $\beta$                                       & $0.1367^{+0.0025}_{-0.0013}$           & -                             \\
% $\log_{10} \rho_0 [\mathrm{g \cdot cm^{-3}}]$ & $-11.70$                               & $-11.78^{+0.18}_{-0.30}$      \\
% $R_\mathrm{D} [R_\mathrm{eq}]$                & $35^{+10}_{-5}$                        & $40^{+10}_{-5}$               \\
% $i\,[\mathrm{^o}]$                            & $43^{+3}_{-2}$                         & -                             \\
% $d\, [\mathrm{pc}]$                           & 49.6                                   & -                             \\
% $E(B-V) [\mathrm{mag}]$                       & -                                      & $0.01^{+0.02}_{-0.01}$        \\
% $n$                                           & -                                      & $2.9 \pm 0.1$                 \\ \hline
% \end{tabular}
% \end{table}
